MI-NeRF: Learning a Single Face NeRF from Multiple Identities

In this work, we introduce a method that learns a single dynamic neural radiance field (NeRF) from monocular talking face videos of multiple identities. NeRFs have shown remarkable results in modeling the 4D dynamics and appearance of human faces. However, they require per-identity optimization. Although recent approaches have proposed techniques to reduce the training and rendering time, increasing the number of identities can be expensive. We introduce MI-NeRF (multi-identity NeRF), a single unified network that models complex non-rigid facial motion for multiple identities, using only monocular videos of arbitrary length. The core premise in our method is to learn the non-linear interactions between identity and non-identity specific information with a multiplicative module. By training on multiple videos simultaneously, MI-NeRF not only reduces the total training time compared to standard single-identity NeRFs, but also demonstrates robustness in synthesizing novel expressions for any input identity. We present results for both facial expression transfer and talking face video synthesis. Our method can be further personalized for a target identity given only a short video.

==> sections/old_experiments.tex <==
\section{Experiments}

\subsection{Dataset and Evaluation}\label{sec:dataset}

\textbf{Dataset.} To evaluate our proposed method, we collected 140 talking face videos of different identities from publicly available datasets~\citep{adnerf,lu2021live,lipnerf,hazirbas2021towards,ginosar2019learning,ahuja2020style,Duarte_CVPR2021,hdtf,wang2021facevid2vid}. We included a variety of standard front-facing videos (e.g.~political speeches), as well as more challenging videos, with large variations in head pose, lighting, and expressiveness (e.g. movies and news satire television programs). The videos are in HD quality (720p) and of around 20 seconds to 5 minutes duration. For each video, we run the 3DMM fitting procedure, as described in Sec.~\ref{sec:input}. We use 100 videos for our training set and we keep the rest as novel identities. 
% \grig{To dataset creation mporei na paei kai se appendix.}

\textbf{Evaluation Metrics.} We measure the visual quality of the generated videos, using peak signal-to-noise ratio (PSNR), structural similarity index (SSIM)~\citep{wang2004image}, and learned perceptual image patch similarity (LPIPS)~\citep{zhang2018perceptual},
and we verify the identity of the target subject, using the average content distance (ACD)~\citep{Vougioukas_2019_CVPR_Workshops,tulyakov2018mocogan}. Additionally, we use the LSE-D (Lip Sync Error - Distance) and LSE-C (Lip Sync Error - Confidence) metrics~\citep{wav2lip,chung2016out}, to assess the lip synchronization, i.e. if the generated expressions are meaningful given the corresponding speech signal.


\begin{table}[t]
\caption{\textbf{Ablation Study.} Quantitative results for different variants of our model. The proposed multiplicative module $M$ leads to the best disentanglement (lower ACD) and visual quality (higher PSNR) with the least possible parameters. }
% The proposed multiplicative module $M_{B}$ enhances the visual quality (higher PSNR).}
\label{tab:ablation}
% \vspace{-10pt}
\begin{center}
\scalebox{0.95}{
\begin{tabular}{|l|c|c|c|c|}
% {|@{\hspace{0.15mm}}l|@{\hspace{0.45mm}}c@{\hspace{0.45mm}}|@{\hspace{0.45mm}}c@{\hspace{0.45mm}}|}
\hline
\textbf{Method} & \textbf{PSNR $\uparrow$} & \textbf{ACD $\downarrow$} & \textbf{LSE-D $\downarrow$} & \textbf{LSE-C $\uparrow$}\\
\hline\hline
Baseline NeRF (without $M$)& 28.65 & 0.229 & 9.08 & 4.06\\
\hline
% (A1) $\bm{W}_1 = \bm{0}$ & 30.17  & 0.16\\
(A1) $M(\bm{e}, \bm{i}) = \bm{W}_{2} \bm{e} + \bm{W}_{3} \bm{i}$ & 29.08 & 0.200 & 8.80 & 4.19 \\
% (A2) $\bm{W}_1 = \bm{I}$ & 30.10 & 0.18\\
(A2) $M(\bm{e}, \bm{i}) = \left(\bm{e} * \bm{i} \right) + \bm{W}_{2} \bm{e} + \bm{W}_{3} \bm{i}$ & 28.84 & 0.207 & 9.07 & 3.80\\
% (A3) $\bm{W}_1 = \bm{W}_2 = \bm{W}_3$ & 29.68  & 0.23\\
(A3) $M(\bm{e}, \bm{i}) = \bm{W}_{1} \left(\bm{e} * \bm{i} \right) + \bm{W}_{1} \bm{e} + \bm{W}_{1} \bm{i}$ & 28.50 & 0.227 & 9.19 & 3.61 \\
% (A4) $\bm{W}_2 = \bm{W}_3 = \bm{0}$ & 31.00 & 0.14\\
(A4) $M(\bm{e}, \bm{i}) = \bm{W}_{1} \left(\bm{e} * \bm{i} \right)$ & 29.12 & 0.228 & 10.49 & 2.36 \\
(A5) $M(\bm{e}, \bm{i}) = \left(\bm{W}_2 \bm{e} \right) * \left(\bm{W}_3 \bm{i} \right) + \bm{W}_{2} \bm{e} + \bm{W}_{3} \bm{i}$  & 28.95 & 0.204 & 9.25 & 3.58 \\
% (A6) $M(\bm{e}, \bm{i}) = \bm{C} \left[ \left(\bm{U}_1 \bm{e} \right) * \left(\bm{U}_2 \bm{i} \right) \right] + \bm{W}_{2} \bm{e} + \bm{W}_{3} \bm{i}$
(A6) $M(\bm{e}, \bm{i}) = \bm{W}_1 \left(\bm{e} * \bm{i} \right) + \bm{W}_{2} \bm{e} + \bm{W}_{3} \bm{i}$
& 28.53 & 0.221 & 9.27 & 3.29 \\
(A7) $M(\bm{e}, \bm{i}) = \bm{\mathcal{W}} \times_2 \bm{e} \times_3 \bm{i} $ & 28.41 & 0.274 & 9.82 & 3.10\\
\hline
\MethodName with $M$ without latent codes $\bm{l}$ & 29.01 & 0.165 & 8.83 & 4.15 \\
\MethodName with $M$ with $k = 32$ & 29.02 & 0.180 & 8.79 & 4.21 \\
\MethodName with $H$ with $N = 4$ & 28.00 & 0.289 & 10.76 & 2.19\\
\hline
\MethodName with $M$ (Ours)  & \textbf{29.73} & \textbf{0.158} & \textbf{8.62} & \textbf{4.24}\\
\MethodName with $H$ (Ours) & 28.95 & 0.180 & 8.82 & \textbf{4.24}\\
\hline
\end{tabular}
}
\end{center}
\vspace{-10pt}
% \vspace{-10pt}
\end{table}


\subsection{Ablation Study}\label{sec:ablation}

We conduct an ablation study on the multiplicative module and the input conditions of \MethodName. Given 10 videos from different identities, we investigate variants of our model (see Table~\ref{tab:ablation}). After training, we synthesize a video of each identity given input expressions from another one. In this way, we evaluate if the model learns to disentangle identity and non-identity specific information.
% , in the most challenging case of two identities (see supplementary).
% We measure the visual quality, using peak signal-to-noise ratio (PSNR), structural similarity index (SSIM)~\citep{wang2004image}, and learned perceptual image patch similarity (LPIPS)~\citep{zhang2018perceptual},
% and we verify the identity of the target subject, using the average content distance (ACD)~\citep{Vougioukas_2019_CVPR_Workshops,tulyakov2018mocogan}.

Firstly, we evaluate the possibility of simply concatenating all the input vectors, as usually done in standard identity-specific NeRFs~\citep{nerface,adnerf,lipnerf}, i.e.~omitting the multiplicative module. We call this ``Baseline NeRF''. As shown in Table~\ref{tab:ablation} and Fig.~\ref{fig:exptrans}, Baseline NeRF cannot learn to disentangle between different identities. It frequently synthesizes a different identity than the target one, or a mixture of identities, based on the identity-expression pairs seen during training.

Variants of the proposed multiplicative module $M$ are examined in rows (A1) to (A7) to determine the simplest and most effective option.
% Interestingly, we found that all three matrices $\bm{W}_{1}$, $\bm{W}{_2}$, and $\bm{W}_{3}$ in Eq.~\ref{eq:multA} need to be distinct and non-zero. This approach allows $\bm{W}_{1}$ to capture the relationship between identity and expression, while $\bm{W}_{2}$ and $\bm{W}_{3}$ capture information from the expression and identity vectors respectively. 
We started by just learning a simple mapping of the $\bm{e}$ and $\bm{i}$ vectors, using $\bm{W}_{2}$ and $\bm{W}_{3}$ matrices (A1). We then explored variants that include a Hadamard product $(\bm{e} * \bm{i})$ to model their non-linear interaction. 
% A simplified version (A5) that employs only $\bm{W}_{2}$ and $\bm{W}_{3}$ results in a decrease in performance, as does (A6), which has fewer parameters and utilizes low rank $\bm{U}_{1} \in \mathbb{R}^{k\times d}$, $\bm{U}_{2} \in \mathbb{R}^{k\times d}$, $\bm{C} \in \mathbb{R}^{d\times k}$, and $k < d$ ($k = 8$ or $k = 32$). We also discovered that our learned $\bm{W}_{1}$, $\bm{W}_{2}$, and $\bm{W}_{3}$ have full rank, indicating that the output $d$ dimension is necessary to capture all the information.
The last variant (A7) is inspired by \citet{wang2019adversarial} and uses $\bm{\mathcal{W}} \in \mathbb{R}^{d\times d\times d}$, requiring significantly more parameters than our proposed $M$ ($d^3$ vs $d^2$). The variant (A6) can be derived from (A7), using similar arguments to \cref{ssec:mi_nerf_app_proof_proposition_multiplicative}. All these variants (A1) - (A7) lead to different disentanglement results, with many of them being quite poor.\looseness-1

In the following rows, we show the small decrease in visual quality if we omit the latent codes, that learn very small per-frame variations in appearance, as noted in Sec.~\ref{sec:input}, or use different hyperparameters: $k = 32$ for $M$ and $N = 4$ for $H$. We conclude that our proposed multiplicative module $M$ leads to the best disentanglement and highest visual quality with the least possible parameters. Our proposed $H$ leads to the second best disentanglement between identity and expression (low ACD metric) and produces videos of comparable visual quality and lip synchronization (LSE metrics).

% The second row of Table~\ref{tab:ablation} shows a small decrease in visual quality if we omit the latent codes. These codes learn very small per-frame variations in appearance, as noted in Sec.~\ref{sec:input}.
% that are necessary to reconstruct in the output videos.

% Variants of the proposed multiplicative module $M$ are examined in rows (A1) to (A7) to determine the simplest and most effective option. Interestingly, we found that all three matrices $\bm{W}_{1}$, $\bm{W}{_2}$, and $\bm{W}_{3}$ in Eq.~\ref{eq:multA} need to be distinct and non-zero. This approach allows $\bm{W}_{1}$ to capture the relationship between identity and expression, while $\bm{W}_{2}$ and $\bm{W}_{3}$ capture information from the expression and identity vectors respectively. 
% A simplified version (A5) that employs only $\bm{W}_{2}$ and $\bm{W}_{3}$ results in a decrease in performance, as does (A6), which has fewer parameters and utilizes low rank $\bm{U}_{1} \in \mathbb{R}^{k\times d}$, $\bm{U}_{2} \in \mathbb{R}^{k\times d}$, $\bm{C} \in \mathbb{R}^{d\times k}$, and $k < d$ ($k = 8$ or $k = 32$). We also discovered that our learned $\bm{W}_{1}$, $\bm{W}_{2}$, and $\bm{W}_{3}$ have full rank, indicating that the output $d$ dimension is necessary to capture all the information.
% The last variant (A7) is inspired by \citet{wang2019adversarial} and uses $\bm{\mathcal{W}} \in \mathbb{R}^{d\times d\times d}$, requiring significantly more parameters than our proposed $M_{A}$ ($d^3$ vs $3d^2$). All these variants (A1) - (A7) lead to different disentanglement results, with many of them being quite poor.
% lead to poor disentanglement \grig{Tha to evaza pio smoothly, typoy "The different models lead to different disentanglement results, with many of them being quite poor, similarly ....".}, producing a different identity or a mixture of identities, similarly to Baseline NeRF (see Fig.~\ref{fig:ablation}).
% We conclude that our proposed multiplicative module $M_{A}$ leads to the best disentanglement with the least possible parameters, while our proposed $M_{B}$ enhances the final visual quality, especially in case of challenging novel expressions.
% In the following sections, we show results of \MethodName with $M_{B}$, denoted as \MethodName for short.

\begin{figure*}[t]
\begin{center}
   \includegraphics[width=\linewidth]{images/expression_transfer.png}
\end{center}
\vspace{-10pt}
   \caption{\textbf{Transferring Novel Expressions.} Qualitative comparison of \MethodName with state-of-the-art approaches for transferring unseen expressions to a target identity. NeRFace~\citep{nerface} is a single-identity NeRF, HeadNeRF~\citep{hong2022headnerf} is a NeRF-based parametric head model, Baseline NeRF concatenates all input conditions, leading to poor disentanglement. Our method demonstrates robustness in synthesizing novel expressions for any input identity.}
\label{fig:exptrans}
\vspace{-10pt}
\end{figure*}

\begin{figure*}[t]
    \centering
\subfloat{\includegraphics[width=0.49\linewidth]{images/time_spk.png}}
\subfloat{\includegraphics[width=0.49\linewidth]{images/psnr_spk.png}}
    % \subfloat[\stl]{\includegraphics[width=0.32\textwidth]{figures/STL10_label_smooth_new.png}}
    % \vspace{-10pt}
    \caption{\textbf{Left:} Training time vs total number of identities. Standard single-identity NeRFs, like NeRFace~\citep{nerface}, AD-NeRF~\citep{adnerf}, and LipNeRF~\citep{lipnerf} require approximately 40 hours training per identity. On the contrary, our \MethodName (generic) can be trained on 100 identities in 80 hours, a $50\times$ improvement over the previous methods. Further personalization takes another 5-8 hours per identity approximately. \textbf{Right:} Corresponding visual quality of generated videos with challenging novel expressions, measured by PSNR (higher the better). Increasing the number of identities improves the robustness of our model to unseen expressions.}
    \label{fig:plots}
    \vspace{-10pt}
\end{figure*}




\subsection{Facial Expression Transfer}

In this section, we demonstrate the effectiveness of \MethodName for facial expression transfer. Given an identity from the training set, \MethodName 
enables explicit control of their expressions, and thus can synthesize high-quality videos of them given novel expressions as input.
% , using different expression vectors as input. \grig{De moy einai poly ksekatharo to task edw.}
% We are particularly interested in challenging novel expressions, not seen for a target identity.
% , which are challenging for the standard single-identity NeRF

\textbf{Results.} Fig.~\ref{fig:exptrans} demonstrates the result of \MethodName with $M$ (personalized) for challenging novel expressions, not seen for the target identity.
% Qualitative and quantitative results are shown in Fig.~\ref{fig:exptrans} and Table~\ref{tab:exptrans}. 
Fig.~\ref{fig:plots} (right) shows the corresponding PSNR, computed on frames with challenging unseen expressions for a particular subject. \MethodName significantly outperforms the standard single-identity NeRFace~\citep{nerface} in such cases. Increasing the number of training identities improves the robustness of our generic model. Further personalization enhances the final visual quality.

Table~\ref{tab:quant} (left) shows the quantitative results of facial expression transfer, computed on 10 synthesized videos (of 10 distinct identities, given a sequence of expressions from a different identity). We compare with methods that similarly allow meaningful control of expression parameters. NeRFace~\citep{nerface} is a standard identity-specific NeRF, without any multiplicative module. Its immediate extension is the Baseline NeRF that is trained on multiple identities, concatenating an additional identity vector as input. HeadNeRF~\citep{hong2022headnerf} is a novel NeRF-based parametric head model, trained on a large amount of high-quality images from multiple identities. 

We notice that NeRFace can produce good visual quality, but cannot generalize to unseen expressions. 
% This is especially true if only a short video clip is used for training, where 
Trained only on a video of a single identity, the model has only seen a limited variety of facial expressions, and thus can lead to artifacts in case of novel input expressions (see second row in Fig.~\ref{fig:exptrans}). Baseline NeRF, as also mentioned in the previous section, leads to poor disentanglement and frequently generates a mixture of identities, depending on the input expression. HeadNeRF distorts the target identity and inaccurately produces the target facial expression. Our method demonstrates robustness in synthesizing novel expressions for any identity, as it leverages information from multiple subjects during training. We encourage the readers to watch the supplementary video.

\textbf{Training Time.} \MethodName significantly outperforms the standard single-identity NeRF-based methods, like NeRFace~\citep{nerface}, in terms of the training time (see  Fig.~\ref{fig:plots} left). Training on 100 identities needs only about 80 hours of training, compared to 40 hours per identity needed by standard NeRFs, leading to a $90\%$ decrease approximately. Further personalization for a target identity adds only another 5-8 hours of training on average, enhancing the visual quality (see Fig.~\ref{fig:plots} right).
% , where we chose challenging novel expressions for an identity to show the difference). 







% Results on test set with fine-tuning on target speaker (short video)

% Training time vs \# identities (without fine-tuning)

% LPIPS vs \#identities (without + with fine-tuning)

% LSE-D vs \#identities (without + with fine-tuning) to measure how accurately the diverse expressions are synthesized

% Figure with unseen/novel expressions (e.g. 4 rows, 2 last unseen/extreme expressions) - cross-identity experiments

\begin{figure*}[t]
\begin{center}
% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=\linewidth]{images/lipsync.png}
\end{center}
% \vspace{-10pt}
   \caption{\textbf{Lip Synced Video Synthesis.} Qualitative comparison of our method with state-of-the-art approaches, GAN-based Wav2Lip~\citep{wav2lip}, AD-NeRF~\citep{adnerf} and Lip-NeRF~\citep{lipnerf}. The original video is in English (1st column). The generated videos (columns 2-5) are lip synced to dubbed audio in Spanish.}
\label{fig:lipsync}
% \vspace{-10pt}
\end{figure*}

\begin{table}[t]
% \vspace{-10pt}
\caption{\textbf{Left:} Facial Expression Transfer. Quantitative comparison of our method with state-of-the-art methods for transferring facial expressions. \textbf{Right:} Lip Synced Video Synthesis. Quantitative comparison of our method with state-of-the-art approaches on generated videos lip-synced to dubbed audio in different languages.}
% \vspace{-10pt}
% \MethodName achieves state-of-the-art performance, trained on multiple identities simulatenously, compared to the single-identity NeRFace~\cite{nerface}.}
% \caption{\textbf{Lip Synced Video Synthesis.} Quantitative comparison of our method with state-of-the-art approaches for generated videos lip-synced to dubbed audio in different languages. The last row corresponds to the original videos, where the lip movements are out of sync with the dubbed audio.}
\label{tab:quant}
\begin{center}
\scalebox{0.85}{
\begin{tabular} %{|l|c|c|c|c|}
{|@{\hspace{0.15mm}}l|@{\hspace{0.45mm}}c@{\hspace{0.45mm}}|@{\hspace{0.45mm}}c@{\hspace{0.45mm}}|@{\hspace{0.45mm}}c@{\hspace{0.45mm}}|@{\hspace{0.45mm}}c@{\hspace{0.45mm}}|}
\hline
\textbf{Method} & \textbf{PSNR $\uparrow$} & \textbf{SSIM $\uparrow$} & \textbf{LPIPS $\downarrow$} & \textbf{ACD $\downarrow$} \\
\hline\hline
NeRFace & 28.11 & \textbf{0.88} & \textbf{0.13} & \textbf{0.11}\\
HeadNeRF & 19.89 & 0.74 & 0.32 & 0.85 \\
Baseline NeRF & 26.21 & 0.85 & 0.22 & 0.32 \\
\MethodName (Ours) & \textbf{28.28} & \textbf{0.88} & \textbf{0.13} & \textbf{0.11}\\
\hline
\end{tabular}
}
\scalebox{0.85}{
\begin{tabular} %{ |l||c|c|c|c|c|c|c| }
{|@{\hspace{0.15mm}}l|@{\hspace{0.45mm}}c@{\hspace{0.45mm}}|@{\hspace{0.45mm}}c@{\hspace{0.45mm}}|@{\hspace{0.45mm}}c@{\hspace{0.45mm}}|@{\hspace{0.45mm}}c@{\hspace{0.45mm}}|}
% @{\hspace{0.45mm}}c@{\hspace{0.45mm}}|}
\hline
\textbf{Method} & \textbf{LSE-D $\downarrow$} & \textbf{LSE-C $\uparrow$} & \textbf{PSNR $\uparrow$} & \textbf{SSIM $\uparrow$} \\
\hline
\hline
AD-NeRF & 11.40 & 1.28 & {27.38} &  {0.84} \\
LipNeRF & {9.92} & {2.71} & {30.10} & {0.89} \\
GeneFace & 11.80 & 2.22 & 25.56 & 0.85\\
\MethodName (Ours) & \textbf{9.46} & \textbf{2.98} & \textbf{30.21} & \textbf{0.90} \\
\hline
% Dubbed & 12.02 & 0.84 & inf & 1.0 & 0.0  \\
%  \hline
\end{tabular}
}
\end{center}
% \vspace{-10pt}
% \vspace{-10pt}
\end{table}

% \begin{table}[t]
% \caption{\textbf{Lip Synced Video Synthesis.} Quantitative comparison of our method with state-of-the-art approaches for generated videos lip-synced to dubbed audio in different languages. The last row corresponds to the original videos, where the lip movements are out of sync with the dubbed audio.}
% % \grig{Ti einai to inf sto dubbed?}}
% \label{tab:lipsync}
% \begin{center}
% % \scalebox{0.8}{
% \begin{tabular} %{ |l||c|c|c|c|c|c|c| }
% {|@{\hspace{0.15mm}}l|@{\hspace{0.45mm}}c@{\hspace{0.45mm}}|@{\hspace{0.45mm}}c@{\hspace{0.45mm}}|@{\hspace{0.45mm}}c@{\hspace{0.45mm}}|@{\hspace{0.45mm}}c@{\hspace{0.45mm}}|@{\hspace{0.45mm}}c@{\hspace{0.45mm}}|}
% \hline
% \textbf{Method} & \textbf{LSE-D $\downarrow$} & \textbf{LSE-C $\uparrow$} & \textbf{PSNR $\uparrow$} & \textbf{SSIM $\uparrow$} & \textbf{LPIPS $\downarrow$} \\
% \hline
% \hline
% % Speech2Vid & 10.97 & 1.71 & 27.67 & 0.84 & 0.26 \\
% % MakeItTalk & 10.23 & 2.21 & 14.15 & 0.25 & 0.39 \\
% % PC-AVS & {8.78} & {3.65} & 14.68 & 0.30 & 0.48 \\
% % Wav2Lip & \textbf{8.06} & \textbf{4.77} & {28.90} & {0.89} & {0.17} \\
% AD-NeRF & 11.40 & 1.28 & {27.38} &  {0.84} & {0.20}  \\
% LipNeRF & {9.92} & {2.71} & {30.10} & {0.89} & \textbf{0.16} \\
% GeneFace &&&& \\
% \MethodName (Ours) & \textbf{9.46} & \textbf{2.98} & \textbf{30.21} & \textbf{0.90} & 0.18 \\
% \hline
% % Dubbed & 12.02 & 0.84 & inf & 1.0 & 0.0  \\
% %  \hline
% \end{tabular}
% \end{center}
% \vspace{-10pt}
% % \vspace{-15pt}
% \end{table}


\subsection{Lip Synced Video Synthesis}

% Results on test set with fine-tuning on target speaker (short video)

% + Comparison with new methods (e.g. GeneFace)

\MethodName can be also used for audio-driven talking face video synthesis, also called lip-syncing. Prior work, LipNeRF~\citep{lipnerf}, has shown that conditioning a NeRF on the 3DMM expression space, compared to audio features, leads to more accurate and photorealistic lip synced videos. Our method naturally extends LipNeRF to multiple identities, using their proposed audio-to-expression mapping.

For this task, we used the dataset proposed by LipNeRF~\citep{lipnerf}~\footnote{We would like to thank the authors of LipNeRF for providing the cinematic data from YouTube.}. It includes 10 videos from popular movies in English, and corresponding dubbed audio in 2 or 3 different languages for each video, including French, Spanish, German and Italian.

% of around 30 seconds to 2 minutes long each in HD resolution (720p). Along with the original audio in English, they collected and aligned the corresponding dubbed audio for each video in 2 or 3 different languages, including French, Spanish, German and Italian. These data are more challenging, due to the cinematic lighting, large head pose variations, emphatic head movements, and expressiveness of the actors.

\textbf{Results. } Table~\ref{tab:quant} (right) shows the corresponding quantitative evaluation of the synthesized videos, lip synced to dubbed audio in different languages. Leveraging information from multiple identities, \MethodName slightly improves LSE metrics and achieves similar visual quality with LipNeRF, at much lower training time (see Fig.~\ref{fig:plots}). AD-NeRF~\citep{adnerf} and GeneFace~\citep{ye2023geneface} lack in lip synchronization for this task.

Fig.~\ref{fig:lipsync} compares the mouth position for two examples, lip synced to Spanish (original audio in English). The GAN-based method, Wav2Lip~\citep{wav2lip}, frequently produces artifacts and blurry results. Since it operates in the 2D image space, it cannot handle large 3D movements. AD-NeRF overfits to the training audio and cannot generalize well to different speech inputs. LipNeRF performs well, but sometimes cannot produce unseen expressions (e.g. does not close the mouth in the first row), since it is only trained on a single video of limited duration. Both AD-NeRF and LipNeRF are standard single-identity NeRFs, requiring expensive identity-specific optimization.
% , compared to our multi-identity NeRF.


\subsection{Short-Video Personalization}

\MethodName can also be adapted to an unseen identity, i.e.~not seen as a part of the initial training set (see Sec.~\ref{sec:personalization}). Fig.~\ref{fig:short} (left) demonstrates the results, when only a very short video of the new identity is available (1 or 3 seconds length). Please note that in this case we use a small number of \textit{consecutive} frames, and thus a very small part of the expression space is covered.
% only a few expressions are seen.
% As described in Sec.~\ref{sec:personalization}, we can fine-tune our network, in order to learn the identity code, given a video of a particular subject. 
In contrast to NeRFace, \MethodName produces satisfactory lip shape and expression, as the multiplicative module has learned information from multiple identities during training. Correspondingly, Fig.~\ref{fig:short} (right) shows the LSE-D metric w.r.t different clip lengths of the target identity for the task of lip-syncing. Since AD-NeRF and LipNeRF are trained on a single identity, they learn audio-lip representations from only 3 or 20 seconds. On the other hand, \MethodName leverages information from multiple identities and leads to a more accurate lip synchronization.
% The single-identity AD-NeRF and LipNeRF can only learn audio-lip representations from a 3 or 20 second video \grig{De katalava ti leei ayti i protasi}, whereas our proposed \MethodName leverages information from multiple identities and leads to a more accurate lip synchronization.


% \textbf{Clip Length. } Fig.~\ref{fig:plots} shows the LSE-D metric w.r.t different clip lengths of the target speaker seen in training. Since AD-NeRF and LipNeRF are trained on a single identity, they learn audio-lip representations from only 3 or 20 seconds. On the other hand, \MethodName learns information from multiple identities, even though the video of the target identity is of only 3 or 20 seconds correspondingly. As a result, \MethodName leads to more accurate lip synchronization.



% Adapt to novel identities - transfer unseen expressions (cross-identity experiments)

% 5, 10, 30, 100, 300, 1000 - shot (consecutive frames, only few expressions seen)

% Figure: progressive improvement

% Diagrams: (1) LSE-D vs \#shots, (2) LPIPS vs \#shots 

\begin{figure*}[t]
\begin{center}
\subfloat{\includegraphics[width=0.49\linewidth]{images/short.png}}
\subfloat{\includegraphics[width=0.49\linewidth]{images/LSE-D_plot_length.png}}
   % \includegraphics[width=\linewidth]{images/short.png}
\end{center}
% \vspace{-10pt}
   \caption{\textbf{Short-Video Personalization.} \textbf{Left:} Qualitative comparison of \MethodName with the single-identity NeRFace~\citep{nerface}, using a video of the target identity of only 1 or 3 seconds duration for adaptation. \textbf{Right:} LSE-D (lower the better) vs clip length of the target identity seen in training, computed on generated videos lip synced to dubbed audio.}
\label{fig:short}
\vspace{-10pt}
\end{figure*}



==> sections/old_intro.tex <==
\section{Introduction}

Capturing the 4D dynamics and appearance of non-rigid motion of humans has long been a challenge for both computer vision and graphics. This task has broad applications, ranging from AR/VR and video games to virtual communication and the movie industry, all of which require the creation of photorealistic videos of the human face. Earlier approaches relied on 3D morphable models (3DMM)~\citep{garrido2015vdub,garrido2014automatic,thies2016face2face}, while more recent methods have turned to generative adversarial networks (GAN)~\citep{pumarola2020ganimation,wav2lip,vougioukas2020realistic}. GANs learn representations of facial dynamics from large datasets, containing video clips from multiple identities. To disentangle latent factors of variation, such as identity and expression, some works have imposed multilinear structures~\citep{wang2019adversarial,georgopoulos2020multilinear}, building on the ideas of TensorFaces~\citep{vasilescu2002multilinear}.
Despite their success, most GANs operate in the 2D image space and they do not model the 3D face geometry. 

Neural radiance fields (NeRF) have recently demonstrated photorealistic 3D modeling of both static~\citep{mildenhall2020nerf,barron2021mipnerf,barron2022mipnerf360} and dynamic scenes~\citep{pumarola2021d,li2021neural,li2022neural}, making them a popular choice for modeling human faces from monocular videos~\citep{nerface,nerfies,park2021hypernerf,rignerf}.
Approaches that leverage a 3DMM prior and condition on expression parameters enable control of facial expressions, for applications such as expression transfer~\citep{nerface} and lip syncing~\citep{lipnerf}. Despite their high-quality results, NeRFs require expensive per-scene or per-identity optimization.
% to capture scene-specific and identity-specific information.
Although some works have learned generic scene representations~\citep{wang2021ibrnet,chen2021mvsnerf,trevithick2021grf,yu2021pixelnerf,kwon2021neural,mu2023actorsnerf}, they require static settings and/or multiple input views during training.


In this work, we propose \MethodName (multi-identity NeRF), a novel method that learns a single dynamic NeRF from monocular talking face videos of multiple identities.
% generalizes dynamic NeRFs to multiple identities.
Using only a \emph{single} network, it learns to model complex non-rigid human face motion, while disentangling identity and non-identity specific information. At the epicenter of our approach lies a multiplicative module that approximates the non-linear interactions between latent factors of variation, inspired by ideas that go back to TensorFaces~\citep{vasilescu2002multilinear}.
% We introduce two possible versions of this module, 
This module learns a non-linear mapping of identity codes and facial expressions, based on the Hadamard product. To the best of our knowledge, this is the first method that learns a single unified face NeRF from monocular videos of multiple identities.

% Our simple architecture can effectively disentangle facial expressions from identity-specific information.
% Since \MethodName is simultaneously trained on videos from multiple identities, it
Trained on multiple videos simultaneously, \MethodName significantly reduces the training time, compared to multiple standard single-identity NeRFs, by up to $90\%$, leading to a sublinear cost curve. Further personalization for a target identity requires only a few iterations and leads to a performance on par with the state-of-the-art for facial expression transfer and audio-driven talking face video synthesis. Since \MethodName leverages information from multiple identities, it also works for very short video clips of only a few seconds length. We intend to release the source code upon acceptance of the paper.
% We additionally show that our method can be extended to other types of deformation, such as human body motion. 

In brief, our contributions are as follows:

\begin{itemize}
    \item We introduce \MethodName, a novel method that learns a single dynamic NeRF from monocular talking face videos of multiple identities.
    \item We propose a multiplicative module to learn non-linear interactions between identity and non-identity specific information. We present two specific parameterizations for this module and provide their technical derivations. 
    % \grig{De moy aresei kai poly ayto: Genika emeis proteinoyme to multiplicative module. Deixnoyme 2 instatiations ayteinoy, oxi oti yparxoyn mono ayta. Diladi kaneis undersell edw. }
    % learns non-linear interactions between latent factors of variation, 
    % \item We achieve up to $90\%$ decrease in training time, while demonstrating state-of-the-art performance for facial expression transfer, talking face video synthesis, as well as human body motion synthesis.
    \item Our generic model can be further personalized for a target identity, achieving state-of-the-art performance for facial expression transfer and talking face video synthesis, requiring only a fraction of the total training time of standard single-identity NeRFs.
\end{itemize}


==> sections/old_related.tex <==
\section{Related Work}

% \grig{Mipws to related work na paei se appendix opws einai? To exw ksanakanei se monostila papers, kai den enoxlise kapoion. Eidika edw poy tha einai akrivws apo katw. Mporoyme na to doyme analoga an exoyme xwro.}
\noindent
\textbf{Human Portrait Video Synthesis.}
Earlier approaches for video synthesis and editing of human faces are based on 3DMMs~\citep{garrido2015vdub,garrido2014automatic,thies2016face2face}. A 3DMM~\citep{blanz1999morphable} is a parametric model that can represent a face as a linear combination of principle axes for shape, texture, and expression, learned by principal component analysis (PCA). 
% These works follow an optimization procedure to get the corresponding parameters for a source and target identity, and then synthesize or reenact them.
More recently, GAN-based networks have been proposed for video synthesis~\citep{kim2018deepvideo,fomm,pumarola2020ganimation}, as well as for audio-driven talking faces~\citep{wav2lip,pcavs,vougioukas2020realistic}. GANs are trained on large datasets with video clips from multiple identities, learning diverse facial expressions and lip movements. However, they operate in a low resolution 2D image space and they cannot model the 3D face geometry. NeRFs~\citep{mildenhall2020nerf} have become very popular, since they can represent the 3D face geometry and appearance, and generate photorealistic videos~\citep{nerface,adnerf,nerfies,park2021hypernerf}.

\noindent
\textbf{Multilinear Factor Analysis of Faces.} Factors of variation, such as identity, expression, and illumination, affect the appearance of a human face in a portrait video. Disentangling those factors is challenging. Techniques like PCA can only find a single mode of variation~\citep{turk1991eigenfaces}. TensorFaces~\citep{vasilescu2002multilinear} is an early approach that approximates different modes of variation using a multilinear tensor decomposition.
% extension of the matrix singular value decomposition (SVD) to tensors. 
Inspired by this, several works have proposed to learn multiplicative interactions to disentangle latent factors of variation~\citep{vlasic2006face, tang2013tensor,wang2017learning}. Multilinear latent conditioning has also been proved beneficial for GANs and VAEs, in order to disentangle and edit face attributes~\citep{sahasrabudhe2019lifting,wang2019adversarial,georgopoulos2020multilinear,chrysos2021conditional}. In this work, we propose a multiplicative module that conditions a NeRF and approximates the non-linear interactions between identity and non-identity specific information.
% \grig{Nomizw oti kai se ayto kai sto apo panw prepei na yparxei mia protasi poy na leei giati den kalyptoyn tin diki mas doyleia, dld oti leitoyrgoyn se mikrotra resolution edw px.}


% \begin{table}[t]
% \begin{center}
% % \begin{tabular}{|l|@{}c@{}|@{}c@{}|@{}c@{}|}  % % tight, no space added.
% \begin{tabular}{|@{\hspace{0.15mm}}l|@{\hspace{0.45mm}}c@{\hspace{0.45mm}}|@{\hspace{0.45mm}}c@{\hspace{0.45mm}}|@{\hspace{0.45mm}}c@{\hspace{0.45mm}}|}
%     \hline
% \textbf{Method} & \textbf{HD Quality} & \textbf{Multiple Identities} & \textbf{Short Clips}\\
% \hline
% \hline
%     GAN & \xmark & \cmark & \cmark \\
%     \hline
%     NeRF & \cmark & \xmark & \xmark \\
%     \hline
%     Ours & \cmark & \cmark & \cmark \\
%     \hline
% \end{tabular}
% \end{center}
% \vspace{-10pt}
% \caption{Current GAN-based approaches for video synthesis of human faces are trained on large datasets of short video clips from multiple identities. In contrast, NeRFs are identity-specific and require long videos for training. Our method combines the HD quality of NeRFs and can be trained on videos from multiple identities of any length.}
% \label{tab:intro_comp}
% \vspace{-10pt}
% \end{table}


\noindent
\textbf{Neural Radiance Fields. }
Implicit neural representations for modeling 3D scenes have recently gained a lot of attention. 
% They are usually based on a deep neural network that maps input coordinates to a signal value, such as signed distance~\citepp{yariv2020idr,wang2021neus,chatziagapi2021sider} or occupancy~\citep{mescheder2019occupancy}. 
In particular, NeRFs~\citep{mildenhall2020nerf,barron2021mipnerf,barron2022mipnerf360,lindell2022bacon} have shown photorealistic novel view synthesis of complex scenes. 
% success in modeling complex scenes and synthesizing photorealistic novel views.
They represent a static scene as a continuous 5D function, using a multilayer perceptron (MLP) that maps each 5D coordinate (3D spatial location and 2D viewing direction) to an RGB color and volume density.
% Using a fully differentiable rendering procedure based on classical volume rendering techniques, the MLP is efficiently optimized to represent the scene. Subsequent works~\citep{barron2021mipnerf,barron2022mipnerf360,lindell2022bacon} propose multiscale representations, attempting to improve NeRF's output visual quality. 
However, NeRFs require expensive per-scene or per-identity optimization.
% In other words, they need to ``overfit'' to a specific 3D scene, in order to capture scene-specific fine details.
A few works have proposed to learn generic representations~\citep{wang2021ibrnet,chen2021mvsnerf,trevithick2021grf,yu2021pixelnerf}, but these require static settings and multiple views as input. In contrast, in this work, we are interested in dynamic human faces, captured from monocular videos.


\noindent
\textbf{Dynamic Neural Radiance Fields for Human Faces. }
Several works have extended NeRFs to dynamic scenes~\citep{pumarola2021d,li2021neural,li2022neural,nerfies,nerface,park2021hypernerf,weng2022humannerf}. They usually map the sampled 3D points from an observation space to a canonical space, in order to learn a time-invariant scene representation. Some additionally learn time-variant latent codes~\citep{nerface,li2022neural,lipnerf}. Particularly challenging is to capture the 4D dynamics and appearance of the non-rigid deformations of the human face from monocular videos.
Conditioning a NeRF on 3DMM expression parameters, related works enable explicit and meaningful control of the synthesized subject~\citep{nerface,adnerf,rignerf,athar2021flame,lipnerf}.
% The learned representation can be then used for applications, like expression transfer~\citep{nerface} and lip-syncing~\citep{lipnerf}.
Although these approaches can produce HD quality results, they are identity-specific and usually require long videos for training.
% have to ``overfit'' to a single identity
Only a limited number of prior works have aimed to train a generic NeRF for human faces~\citep{raj2021pixel,hong2022headnerf,zhuang2022mofanerf}. However, all of these models require multiple views for training. In contrast, we propose a simple architecture that is capable of learning multiple identities from monocular talking face videos of arbitrary length captured in the wild.


% \noindent
% \textbf{Generic Neural Radiance Fields for Humans.}
% Only a limited number of prior works have aimed to train a generic NeRF for human modeling~\citep{raj2021pixel,hong2022headnerf,zhuang2022mofanerf,kwon2021neural,mu2023actorsnerf}. However, all of these models require multiple views for training.
% Both HeadNeRF~\citep{hong2022headnerf} and MoFaNeRF~\citep{zhuang2022mofanerf} are parametric models, and thus limited to approximating a target subject based on the available training distributions. 
% that rely on complex convolutional networks to enhance their output quality. They are limited to approximating a target subject based on the available training distributions. In contrast, we propose a simple architecture that is capable of learning multiple identities from monocular videos captured in the wild, and can synthesize high-fidelity animations for them.


